Hidden Classification Layers: Enhancing linear separability between classes in neural networks layers

In the context of classification problems, Deep Learning (DL) approaches represent state of art. Many DL approaches are based on variations of standard multi-layer feed-forward neural networks. These are also referred to as deep networks. The basic idea is that each hidden neural layer accomplishes a data transformation which is expected to make the data representation "somewhat more linearly separable" than the previous one to obtain a final data representation which is as linearly separable as possible. However, determining the appropriate neural network parameters that can perform these transformations is a critical problem. In this paper, we investigate the impact on deep network classifier performances of a training approach favouring solutions where data representations at the hidden layers have a higher degree of linear separability between the classes with respect to standard methods. To this aim, we propose a neural network architecture which induces an error function involving the outputs of all the network layers. Although similar approaches have already been partially discussed in the past literature, here we propose a new architecture with a novel error function and an extensive experimental analysis. This experimental analysis was made in the context of image classification tasks considering four widely used datasets. The results show that our approach improves the accuracy on the test set in all the considered cases.

==> SEC_RELATED_WORKS.tex <==
\label{sec:related}
In \citep{lee2015deeply} a similar approach was proposed. However, the supervision of the hidden layer was made by SVMs instead of neural networks, affecting the construction of the proposed final loss. Instead, in this proposed work a standard ANN hidden layer as supervisors is used, not requiring the adoption of specific loss functions.% allowing simple combinations of classical loss functions to train the complete model.  

In \citep{wang2020cascade} a cascade CNN (C-CNN) is proposed. The aim is to avoid the information loss caused by consecutive convolution striding or pooling in a motor fault diagnosis task. The proposed network is composed of a CNN having the outputs of the first hidden layers combined together through  dilated convolutions and trained using a proposed progress optimization algorithm. 

\roberto{Questa parte è da allargare ed approfondire}

==> latexmkrc <==
$pdflatex = 'pdflatex --halt-on-error %O %S';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
